Korali: Efficient and Scalable Software Framework for Bayesian Uncertainty Quantification and Stochastic Optimization

We present Korali, an open-source framework for large-scale Bayesian uncertainty quantification and stochastic optimization. The framework relies on non-intrusive sampling of complex multiphysics models and enables their exploitation for optimization and decision-making. In addition, its distributed sampling engine makes efficient use of massively-parallel architectures while introducing novel fault tolerance and load balancing mechanisms. We demonstrate these features by interfacing Korali with existing high-performance software such as Aphros, Lammps (CPU-based), and Mirheo (GPU-based) and show efficient scaling for up to 512 nodes of the CSCS Piz Daint supercomputer. Finally, we present benchmarks demonstrating that Korali outperforms related state-of-the-art software frameworks.

==> figures/korali_conduit_parallel.tex <==
% We need layers to draw the block diagram
\pgfdeclarelayer{background}
\pgfdeclarelayer{foreground}
\pgfsetlayers{background,main,foreground}

% Define a few styles and constants
\tikzstyle{subModule}=[draw, fill=blue!20, text width=5em, text centered, minimum height=2.5em]
\tikzstyle{module} = [subModule, text width=6em, fill=red!20, minimum height=12em, rounded corners]
\tikzstyle{worker} = [draw, fill=orange!50, text width=5em, text centered, minimum height=3.5em]
\tikzstyle{rank} = [draw, fill=orange!50, text width=5em, text centered, minimum height=1.15em]
\tikzstyle{model} = [draw, fill=green!10, text width=7.2em, text centered, minimum height=3.5em]
\def\blockdist{2.3}
\def\edgedist{2.5}

\tikzstyle{doc}=[%
draw,
thick,
align=center,
color=black,
shape=document,
minimum width=7mm,
minimum height=13.2mm,
shape=document,
inner sep=2ex,
]

\begin{tikzpicture}
    
       %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    % Drawing static korali objects
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    
    % Drawing Conduit
    \node (conduit) [module, minimum height=17em]{\textbf{Distribution Conduit}};
    \path (conduit.center)+(0,2.0) node (distributeSamples) [subModule] {Distribute Samples};
    \path (conduit.center)+(0,-2.0) node (collectResults) [subModule] {Collect Results};
    
    % Drawing workers
    \pgfmathsetmacro{\n}{3}
    \foreach \i in {1,...,\n}
    {
      \path [draw, ->] ([xshift=-30pt, yshift=-12 + \i*4.0pt] distributeSamples.west) -- ([yshift=-12 + \i*4.0pt] distributeSamples.west);
      \path [draw, ->] ([yshift=-12 + \i*4.0pt] collectResults.west) -- ([xshift=-30, yshift=-12 + \i*4.0pt] collectResults.west);
      
      \path (conduit.east)+(2.4, +3.8 - \i*1.6) node (worker\i) [worker] {\textbf{Worker \ifthenelse{\i=3}{k}{\i}}};
      
      \ifthenelse{\i=3}{\path (worker\i.north east)+(0,0.4) node (manyWorkers) {$\vdots$};}{}
      
      \path (worker\i.north east) node[anchor=north west] (rank_\i_0) [rank] {\scriptsize{Rank 0}};
      \path ([yshift=1pt] rank_\i_0.south) node[anchor=north] (rank_\i_1) [rank] {\scriptsize{...}};
      \path ([yshift=1pt] rank_\i_1.south) node[anchor=north] (rank_\i_m) [rank] {\scriptsize{Rank $m$}};
      
      %\path [draw, ->] (distributeSamples.east) to [out=-10*\i + 5, in=180 - 3*\i] node [xshift=10 +  \i*1, yshift=32 - \i*16] (sampleSetTitle\i)
      %{\ifthenelse{\i=3}{$S'_{k}$}{$S'_{\i}$}} (worker\i.west);
      \path [draw, ->] (distributeSamples.east) to [out=-10*\i + 5, in=180 - 3*\i] node [xshift=10 +  \i*1, yshift=32 - \i*16] (sampleSetTitle\i)
      {} (worker\i.west);
      
      \path (rank_\i_1.east) node[anchor=west] (model\i) [model] {\textbf{Computational Model} $f$ };
      \path (collectResults.center)+(225 -\i*4.3pt,-0.58 + 0.2*\i) node (collectPreNodeA\i) {};
      \path [draw, -] (model\i.south)+(-\i*3.9pt,0) -- (collectPreNodeA\i.east) node {};
      
      \path [draw, ->] (collectPreNodeA\i.east) -- ([yshift=-14 + \i*5.0pt]collectResults.east);
    }

    \path (distributeSamples.west)+(-1.0, -0.75) node (resultsText) {$\{S'_i\}_{i=1}^n$};
    \path (collectResults.west)+(-1.0, -0.75) node (resultsText) {$\{f(S'_i)\}_{i=1}^n$};
    \path (collectPreNodeA3)+(-1.0, -0.75) node (resultsText) {$f(S'_{1}), \, f(S'_{2}), \, ..., \, f(S'_{n}), \, $};
 
    
\end{tikzpicture}


==> figures/pipe/download_daint <==
#!/bin/bash

set -eu

: ${base=daint:/scratch/snx3000/karnakov/bubblePipe}

e () {
  echo "$@"
  eval "$@"
}

getname () {
  echo $1 | sed -En 's|.*result([^/]*)/(gen...)/(sample......).*|\1_\2_\3|p'
}

frame=a_0042.png
# dumpdt=0.05
# width=0.15
# t=frame*dumpdt/width

copy () {
  path=$base/$1
  name=${2:-$(getname $path)}
  e "rsync -zzaPL '$path/vis/$frame' '${name}.png'"
  e "rsync -zzaPL '$path/objectives' '${name}.objectives'"
}

copy resultMaxMeanVel/gen141/sample000001
copy resultMaxNumCoal/gen150/sample000000
copy resultMinNumCoal/gen151/sample000000
copy pipe_baseline baseline

